PIANIST: Learning Partially Observable World Models with LLMs for Multi-Agent Decision Making

Effective extraction of the world knowledge in LLMs for complex decision-making tasks remains a challenge. We propose a framework PIANIST for decomposing the world model into seven intuitive components conducive to zero-shot LLM generation. Given only the natural language description of the game and how input observations are formatted, our method can generate a working world model for fast and efficient MCTS simulation. We show that our method works well on two different games that challenge the planning and decision making skills of the agent for both language and non-language based action taking, without any training on domain-specific training data or explicitly defined world model.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We outline the scope of our paper and include the main contributions and claims in the abstract and introduction, including details on what our method is and what settings we tested our method in.
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We include a limitations section (section \ref{sec:limitations}) in the paper where we reflect on our experimental setting and whether it generalizes to other settings as well. We discuss how more agents increases the noisiness of the feedback. 
    % We also discuss how our method scales. 
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}
    % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not include any theoretical results
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We disclose all the information needed to implement our method, including detailed pseudocode [\ref{alg:method_pseudocode}], diagrams [\ref{fig:agentframework}, \ref{fig:skillcoach}], and sections in the appendix with more detailed information about our implementation[\ref{sec:avalon_agent},  \ref{sec:dialogue_gen_anal}, \ref{sec:dialogue_guide_improve}]
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We will open source the codes along with detailed instructions for reproducing the experimental results in this work.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We specify what games we play on, how many functions we generated, etc in the paper. For example, for the improvement process we show these parameters above table \ref{tab:evolver} in the caption. 
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We report necessary error bars for statistical significance, see e.g., Table~\ref{tab:evolver}, Table~\ref{tab:rl_evolver}, Table~\ref{tab:feedback}, Figure~\ref{fig_gpt_4_35}, Figure~\ref{fig_avalon_gops_rl_improve}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We summarize our experiment compute resource in Appendix~\ref{append_exp_comput_src}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have read ethics guidelines and have checked that our paper conforms to the  NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  Our paper is foundation research and does not have a direct path to negative applications. 
    % s suchOur paper does not involve any of the impacts mentioned
    % We have discussed both  positive societal impacts and negative societal impacts of our work in this paper that are relevant.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not scrape any data nor do our models pose high risk for misuse.
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We cite and credit all the previously published work that we have mentioned in this paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not release new assets. All our data is self-generated.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not involve human subjects. Only AI ones.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  We do not involve human subjects. Only AI ones.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}


==> sections/conclusion.tex <==
\section{Conclusion}

==> sections/directions.tex <==
\section{Methodology}

% In relation to improving the adaptability and reasoning capabilities of LLM agents, we believe the following directions to be of key interest. 

As discussed in the introduction, many approaches leverage inherent structure in the domain of the problem to achieve better performance. Some methods leverage the fact that it is easy to check for correctness. Other methods leverage the step-by-step nature of the problem, where the problem can be naturally divided into steps. In our particular case, 

We want to develop LLM agents that are able to leverage these inherent problem structures without further guidance from humans. In other words, the LLM agent should, through self improvement, be able to figure out by itself what structures of the problem are useful, and how to conduct search for this specific problem. In the context of games, this means that the LLM agent should be able to, given the rules of the game in natural language, understand and zero or few shot play the game well. Humans are able few shot play Avalon well given the rules of the game, so we want to develop LLM agents that can also do this.

There are a couple of key ingredients that are necessary to construct such an LLM-agent able to play Avalon, which we discuss in more detail below. We believe there are many interesting areas to improve on in each of the core components. 

\subsection{Policy model}

A good policy model will be able to reason and plan ahead, as well as produce good actions with few examples from the domain. Usually, in the world of LLM agents, a good policy model will incorporate some form of step-by-step reasoning (chain of thought), which helps the LLM reason through problems (\cite{wei2022chain}). This could be in the form of $k$-beam search, where we take the best $k$ actions at each step and propagate them further down the chain. $k$-beam search tends to be a good, computationally efficient baseline. It could also be in the form of a tree, like in tree of thought (\cite{yao2023tree}), where we branch out all of the actions. Branching out all the actions is obviously very computationally intensive.

Of particular interest to us here will be using search techniques to guide the search process across the steps smartly so that we do not have to branch out to everything. Search techniques have shown great promise in areas that require deep strategic thinking, such as MCTS in go (\cite{silver2017mastering}). MCTS with LLMs have already shown great promise in next token prediction in code generation (\cite{zhang2023planning}), and is a good benchmark. Essentially what MCTS does is it selects which nodes to expand in the search tree based on the probability of getting there and the expected exploitation and exploration value of that state. We hope to adapt search techniques such as MCTS with tree of thought prompting to allow for planning over more abstract states than just tokens. 

We believe that using the LLM to guide the search process will lead to more efficient and effective search. For instance, when determining which states to expand, an LLM can, using its world knowledge, help choose which one is most promising. This will massively reduce the computation time for tree based search approaches, which can be exponential in the number of actions and search depth. Moreover, in settings with adversarial actors, such as in games, we can use traditional game theoretic techniques such as alpha-beta pruning to further reduce the computational burden.

More specifically, we adapt a MCTS framework similar to that of MuZero (\cite{schrittwieser2020mastering}). In MuZero, three separate models are trained to guide the MCTS process: (1) a representation model, (2) a dynamics model, and (3) a prediction model. We aim to do something similar, but where these models are generated by the LLM. There are two ways in which the LLM can do this. The first way is to prompt the LLM each time we want to predict something during the search process. However, this process is incredibly computationally intensive. The second, and much more feasible way is to have the LLM generate a function, usually in code, that we can use as one of the three models. This way we only need to call the LLM when we generate the function. We elaborate more on how to have the LLM learn and generate better functions in the learning section below. Given the simplicity of the action rules for Avalon, we suspect that the dynamics model and state evaluator will not be too hard to generate. However, predicting the policies of all the players might present a significant challenge, especially given the hidden information nature of the game. 

\subsubsection{Language and Action}

An important difference between social deduction games such as Avalon and Go is that Avalon has a heavy discussion and dialogue component. While what you speak does not directly affect the outcome of the game (the discussion in Avalon is cheap talk), you can still influence other players and receive useful information from dialogue. 

There have been studies of developing agents that are able to play games with both dialogue and actions well. Diplomacy is an example of such a game where researchers developed a landmark AI agent called Cicero (\cite{gray2020human}). However, note that there are a couple of key differences between their study and ours. Firstly, dialogue, deduction, and deception play a far greater role in Avalon than in diplomacy. Diplomacy is more focused on actions, and honest, trustworthy behavior can often allow you to build solid alliances and win the game. In fact, there are a few modes in Diplomacy where dialogue is not allowed. Secondly, Cicero does not use LLMs, and it does not few-shot play the game. Cicero is trained on comprehensive gameplay data taken from Webdiplomacy, the diplomacy playing website.  

However, there are still many techniques from Cicero that we can adapt to our Avalon playing agent. Cicero roughly has three key component models: (1) a natural language generation model (2) a natural language understanding model and (3) a strategic reasoning model. The natural language understanding model takes dialogue from other players as input, and predicts the players intent (i.e. what actions they are likely to take next based on what they say). The strategic reasoning model then takes this information, along with the game state, to produce action intents. Given the action intent produced by the reasoning model along with the previous dialogue, the natural language generation model then produces dialogue that aligns with the action intent. Planning over natural language space is incredibly hard since the action space for natural language is infinite. Hence, what Cicero essentially does is it extracts action intents from dialogue and plans over intents instead.

We can do something similar in Avalon, but where we use an LLM instead of training a new language model. We can also extract action intents in Avalon by simply asking the LLM to generate intents for each player based on the discussion. Then we can use MCTS over the intent state and action space instead of natural language space, hence dramatically reducing the number of states we need to search. More specifically, we factor the observed intent of the players into what actions they are likely to take during the MCTS search process. We then ask the LLM to generate dialogue based on the optimal series of actions produced by MCTS. By intent, we can analyze several things, including (1) what next actions they are likely to take, such as voting (2) what secret role they have and (3) what beliefs they hold about other players. When human players play Avalon, they usually think and reason through such intents, so we think LLM-agents will perform well if they do so too. All three of these types of intents are also commonly seen in other tasks where we need to figure out the motives of other players. 

We elaborate more on how specifically actions and dialogue are generated in the implementation section.

\subsection{Functional Value/Reward model}

A good reward model is crucial in aligning the agent towards good behavior in the domain. In some domains a reward model is concretely defined beforehand, perhaps in the form of a verifier for code correctness for example. In other domains with more abstract rewards, such as chatbots, RLHF is commonly used, where a separate reward model is trained on the training data, and kept frozen as we use it to align the pre-trained model to the domain. However, in domains with little training data, training the reward model itself becomes an obvious challenge. Foundation models, with their world knowledge, can also help us create a reward model from little data here -- for example we can use LLMs as a reward model to score the responses based on some predefined domain specific criteria defined in natural language.

The reward model can also be trained along with the policy model. In fact, it seems that an adaptive, self-improving reward model seems to perform better than a static one. We will see an example of an adversarial reward network in the next section, in which the learning for the policy and reward networks are strongly integrated together -- they can use the same loss function in fact. We mention briefly a non-adversarial example of using an LLM as a judge for now, where the same LLM is used as both the policy model and reward model (\cite{yuan2024self}). The LLM is given some predefined criteria as a prompt before scoring. After generating and scoring using the same model, preference pairs are selected and DPO is used to train the model on how well it performs as a policy model. Note that the reward model is not explicitly trained here, though it does change over time. 

Another key consideration when training a reward model is what parts of the response do we train it on. For example, if we are using CoT reasoning on a math problem, do we just train the reward model on whether the answer is correct, or do we also judge the intermediate steps? \cite{lightman2023let} investigate this problem by training an outcome based reward model (ORM) and a process based reward model (PRM) based on human annotated feedback. Indeed, as the common human adage suggests, we should `focus on the process not the outcome,' and they found that the PRM is significantly better and more aligned than the ORM. However, a weakness of process supervision is that it can often be more training data intensive than outcome supervision.

In our application, if we have the LLM generate functions, we want to evaluate how good the generated functions are. If we have access to a game simulator, we can try comparing outputs of the generated function with that of random rollout to score the function. If we do not have a simulator, we will need to score based on (1) the actual game play, (2) the internal world model of our agent, or (3) some trained reward model. Note that the internal world model of the agent may be configured to allow for internal simulations, such as in the case of MCTS. 


We can also use an LLM as a reward model, where we have the LLM score the generations based on some criteria and rules. After critiquing the generations, the LLM can then suggest improvements. We will see an example of this in the next section. 

\subsection{Learning algorithm}

% Given an appropriate reward model, we can generate synthetic training examples using the policy model, and generate more samples as we train like in reinforced self-training (ReST) (\cite{gulcehre2023reinforced}). This training process is very similar to online reinforcement learning, where new data is generated as we take actions based on the policy model, and the policy model is then trained on the new data. Hence, the training sample is not i.i.d. anymore, but rather is \emph{dependent} on the policy model. Unlike traditional online approaches, however, in ReST the size of the grow and improve steps can be controlled, i.e. we can adjust how many times we tune the model per data generation step, thus improving the computational efficiency of learning. We can also use filtering techniques to gradually refine the data generated as we train, which results in better learning over time. However, a weakness with this approach is that it requires a reward model that is both well aligned on the training data and on the new synthetic data. 

\subsubsection{Evolutionary improvement}

LLMs can generate very different responses under the same prompt, especially when we are generating long responses such as functions. We can leverage this to our advantage, because the randomness allows us to explore across a couple of options and choose the best one. In fact, we have already observed great variability in the performance of value functions generated on simpler games such as GOPS. Using this variability, we can then explore and develop on different options.

One simple way to do this is to keep track of the $k$-best generated functions, similar to beam search. The self-improvement process is divided into two parts -- improvement and scoring. During the scoring step, all the generated functions are scored, and the $k$ best functions are stored. During the generation step, we ask the LLM to suggest possible improvements upon the $k$ best functions. We then feed these possible improvements to the scoring step, and repeat the process of self improvement. 

This process has shown great promise in prior literature. In Eureka, for example, researchers used evolutionary improvement to create a good reward function (reward engineering, reward shaping), which is then used to train an RL agent to perform tasks such as pen spinning and walking (\cite{ma2023eureka}). Specifically, there are three components to their process: (1) an environment as context that allows for zero-shot generation of executable reward functions, (2) an evolutionary search process similar to the one we described, and (3) reward reflection. 

They first feed the environment source code to a coding LLM and asks it to generate a reward function in python given the environment semantics. They then sample from the LLM and filter out buggy functions (usually the ratio is 16 buggy functions to 1 executable function). Then, based on the initially generated functions, at each improvement step, the LLM proposes a new improved function (i.e. mutation) from one of the best performing function from the previous iteration using textual feedback (\cite{ma2023eureka}). The textual feedback usually includes suggestions on ways to change the existing reward function. This is generated through reward reflection, where policy generated using the corresponding reward function is evaluated on the environment, and all the intermediate values of the components of the reward function are recorded down so that we can better keep track of what part of the reward function needs improvement. 

We can do something similar. While we might not have a direct way to measure the quality of the trained policy like in Eureka, we can still run simulations of how policy performs using either an external simulator or internal one, for both the environment and the opponent. Then, we can use a similar approach where we break down the various components of the reward function and provide feedback based on that. 



% \subsubsection{Adversarial Training}

% % adversarial fine tuning

% Learning can also be done adversarially. For example, we can fine tune a LLM through adversarial self-play (\cite{chen2024self}). Specifically, in a learning process very similar to generative adversarial networks (GANs) in computer vision, the same LLM is used both as a generator, to generate human like responses to the prompt, and a discriminator (or reward model, scoring function), to distinguish between human responses and synthetic responses from the generator. 
% If $f$ is the discriminator, with $f(x,y)$ being how likely the discriminator that the response $y$ is generated by humans given prompt $x$, the loss function for discriminator becomes
% \[\mathbb{E}_{x \sim q(\cdot), y \sim p_{\text{data}}(\cdot|x), y' \sim p_{\theta}(\cdot|x)} \left[ \ell \left( f(x, y) - f(x, y') \right) \right]
% \]
% where $\ell$ is some convex function, and that for the generator becomes
% \[\mathbb{E}_{x \sim q(\cdot), y \sim p(\cdot|x)} \left[ f_{t+1}(x, y) \right] - \lambda \mathbb{E}_{x \sim q(\cdot)} \left[ KL \left( p(\cdot|x) \parallel p_{\theta}(\cdot|x) \right) \right]
% \]
% where we have an additional regularization term. 
% The model is then updated simultaneously using the combined losses of both the discriminator and generator in an online fashion. Presumably, training a the LLM to be a better discriminator encourages it to better utilize its world knowledge about the domain. Hence, the key difference between the adversarial and non-adversarial settings is that the `reward' model in the adversarial setting is adaptive to the generator.

% Adversarial training will be particularly relevant in game settings, since games typically involve adversaries. In game settings, it is easy for the agent to experience mode collapse and generate the same strategy that an opponent can easily adapt to. 

% One way we can adversarially improve the functions that the LLM generates is by having an adversarial LLM come up with counter examples where the generated function does not work well. 

\subsubsection{Curriculum learning}
% curriculum learning

As seen in some of our previous discussions, the order in which you feed model training data also matters a lot in training. For example, we saw how in ReST, we gradually filter out more and more `low quality' training data, resulting in better performance. This is commonly known in the research community as curriculum learning. It is not hard to imagine how one could also use an adversarial curriculum, where we deliberately choose examples that the policy model performs poorly on to quiz it and help it learn better.

Eureka has used curriculum learning to great effect in training a hand to spin a pen (\cite{ma2023eureka}). Specifically, they train the hand on manageable components such as re-orienting the pen, completing a sequence of configurations, etc. We can do something similar with the dialogue generation in Avalon by training the language component on skills such as deduction, deception, and negotiation independently. 

% group learning 


% \subsection{Tool Usage}
% Many domains that LLM-agents are deployed in require some usage of external tools, whether this be web-browsing or some interface to run generated code on. Tools can also enhance the ability of the LLM to generate better NLP responses -- for example, and LLM-agent doing job scheduling could benefit from having access to a schedule optimizer, or the ability to run optimization algorithms.

% In Avalon, if the LLM is generating functions, the obvious tool that LLMs such as ChatGPT have access to is a code running environment. They could run and test their generated function by themselves. 

% We want to develop LLM-agents that are able to use tools more effectively, and moreover, learn how to use tools. The LLM-agent should be able to figure out what is the best tool to use in this domain through self improvement. 




==> sections/impact.tex <==
\section{Applications}
A LLM Agent able to learn through self-improvement will greatly enhance the application of LLMs to different domains, automatically tasks that are impossible to train on given either the scarcity of the data or the dependency of the data on actions taken. We list some potential applications below.

\subsection{Dialogue systems}
Dialogue systems are a very natural application of LLM-agents, since many LLMs are already pretrained to be chatbots, and many dialogue systems operate under niche domains where data is scarce. An example of this is a customer support bot, which is very domain specific to the product it is helping with. Moreover, the support bot also needs to reason about what the customer needs, and what the best solution is to the problem. For a LLM-agent to achieve this, it will require many of the methods we hope to investigate. 
\subsection{Code generation}
Code generation is another very natural application of LLM-agents. LLM agents can already generate functional code given a prompt, and have a great grasp of syntax in coding. However, there are many tasks which cannot yet be automated by LLMs. For example, debugging -- the programmer's bane -- is something that can be automated by LLM-agents. LLM-agents can already call upon programming tools such as an interactive coding environment. It is not hard to imagine that  it can also run experiments to debug code or use debugging tools available. 




\subsection{LLM Summarization and Representation Learning}
As we know, LLMs are able to perform the important function of summarizing text such as conference papers. While LLMs have been demonstrated to perform on par with humans even on tasks with more practical applications (\cite{yang2023exploring}), it is important to note that evaluation of these summaries on subsequent downstream tasks have not been well explored. 

% As we know, the quality of the output from a LLM is highly dependent on the quality of the prompt.

For example, a LLM-agent providing legal advice might be provided hundreds of documents to read in order to determine whether a certain action is legal or not. The finite context window means that obviously we cannot feed the LLM the entire drawer of documents. Moreover, the summary should only provide information that is relevant to deciding whether the action is legal or not. 

In many practical applications, summarization is an intermediate step towards some subsequent task, whether it be travel advice or debugging tips.  Thus, summarization can be thought of as an encoder on the space of natural language, and training a LLM to summarize better is equivalent to representation learning. The downstream task can be completed by a human, another model, or even another LLM. In fact, adding an intermediate summarization step can make LLMs perform reasoning tasks better!

Research in representation has shown that certain representations are better than others. Specifically, the properties of disentanglement , completeness, and informativeness seem to be particularly useful (\cite{eastwood2022dci}), as well as invariance when it comes to downstream reinforcement learning applications (\cite{zhang2020learning}). We believe that similar representation learning techniques and qualities can be applied towards improving LLM summarization for downstream tasks.


% \subsection{Automated negotiation}
% TBD



==> sections/limitations.tex <==
% \section{Limitations}
% \label{sec:limitations}

% While our method performs better on average, individual runs can have high variance. 
% Since the performance of an agent in multi-agent adversarial game settings is highly dependent on opponents' policies, feedback from these environments tend to be highly noisy, with noise increasing with the number of players.
% This is especially true when learning Avalon heuristics, where the performance depends on the policies of 5 other players, teammates and opponents. 
% We believe that running more game simulations with different opponent policies can help reduce this feedback noise. We also acknowledge the inherent noisiness in LLM generations and how that can impact our results. We tried to reduce this noise by (1) using the same seed functions when benchmarking the different LLM improvement methods and (2) collecting generated strategies from multiple runs. 
% We also did not test our method on other non-adversarial environments such as question answering and text-based worlds. 
% However, given the strong performance of our method in adversarial multi-agent settings, we believe that similar performance will be observed in single agent, non-adversarial  settings. 

\section{Conclusion}
In conclusion, we have presented \method, a generalizable, training-free method of integrating search methods with large language models to create an embodied agent capable of advanced planning and decision making. 
The strong zero-shot performance of such an agent, \emph{without any domain specific training}, on complex decision and planning tasks such as GOPS and Avalon suggests the power of such approaches towards creating generalized agents. 
